A holistic look at requirements engineering practices in the gaming industry

In this work we present an account of the status of requirements engineering in the gaming industry. Recent papers in the area were surveyed. Characterizations of the gaming industry were deliberated upon by portraying its relations with the market industry. Some research directions in the area of requirements engineering in the gaming industry were also mentioned.

==> Makefile <==
## -*- mode: Makefile -*-
##
## This is a sufficient `Makefile', but not a great one.
##
## "Normal" PDF is generated via `pdflatex'.  This is the route you take if you
## make `<doc>.pdf'.
##
## "Alternative" PDF can be generated via `dvips' and `ps2pdf'.  This is the
## route you take if you make `<doc>-ps.pdf'.
##

###############################################################################

# The root documents, minus their `.tex' file name extensions.  Each of these
# is a (phony) Make target.  The first root file listed in `DOCUMENTS' is the
# default target.
#
DOCUMENTS	:= main
DOC		:= $(firstword $(DOCUMENTS))

# "Extra" figures, not made by xfig, inkscape, or gnuplot.  These must have
# file name extensions because we don't want to infer them.
#
EXTRAFIGEPS	:=
EXTRAFIGPDF	:=
EXTRAFIGWWW	:=

# The files that we are required to submit: a PDF file and a LaTeX "paper
# metadata" file.  (Sheridan now longer requests a PS file; hooray!) See the
# VEE 2016 instructions to authors, in the `etc' directory.
#
VEE_ROOT	:= vee49-burtsev
VEE_PDF		:= $(VEE_ROOT).pdf
# VEE_PS	:= $(VEE_ROOT).ps
VEE_TEX		:= $(VEE_ROOT).tex

###############################################################################

TEXINPUTS	:= .:./figs::
BIBINPUTS	:= .::

export TEXINPUTS
export BIBINPUTS

LATEX		:= latex
PDFLATEX	:= pdflatex
BIBTEX		:= bibtex

DVIPS		:= dvips
PS2PDF		:= ps2pdf14
FIG2DEV		:= fig2dev
INKSCAPE	:= inkscape
GNUPLOT		:= gnuplot
#
# For producing the VEE '16 submission package...
# PDFTOPS	:= pdftops
M4		:= m4
CP		:= cp

PDFLATEXFLAGS	:= -interaction=nonstopmode -halt-on-error -file-line-error

# See below for some long-winded comments about these options.
#
DVIPSFLAGS	:= -Ppdf -Pcmz -Pdownload35 -u ps2pk.map -tletter -G0
PS2PDFFLAGS	:= -sPAPERSIZE=letter -dPDFSETTINGS=/printer \
		   -dColorConversionStrategy=/RGB \
		   -dProcessColorModel=/DeviceRGB \
		   -dEmbedAllFonts=true -dSubsetFonts=true -dMaxSubsetPct=100
PS2PDFFLAGS_EPS	:= -dEPSCrop -dPDFSETTINGS=/printer \
		   -dColorConversionStrategy=/RGB \
		   -dProcessColorModel=/DeviceRGB \
		   -dEmbedAllFonts=true -dSubsetFonts=true -dMaxSubsetPct=100

TEX4HT		:= tex4ht
T4HT		:= t4ht

# TEXBITS	should exclude the root files, but it does not.
TEXBITS		:= $(filter-out $(VEE_TEX),$(wildcard *.tex))
BIBBITS		:= $(wildcard *.bib)

FIGBITS		:= $(wildcard figs/*.fig)
SVGBITS		:= $(wildcard figs/*.svg)
PLOTBITS 	:= $(wildcard plots/*.gnu)
FIGEPS		:= $(FIGBITS:.fig=.eps) $(SVGBITS:.svg=.eps) \
		   $(PLOTBITS:.gnu=.eps) \
		   $(EXTRAFIGEPS)
FIGPDF		:= $(FIGBITS:.fig=.pdf) $(SVGBITS:.svg=.pdf) \
		   $(PLOTBITS:.gnu=.pdf) \
		   $(EXTRAFIGPDF)
FIGWWW		:= $(FIGBITS:.fig=.png) $(SVGBITS:.svg=.png) \
		   $(PLOTBITS:.gnu=.png) \
		   $(EXTRAFIGWWW)

DEPS		:= $(wildcard *.cls) $(wildcard *.sty) $(wildcard *.cfg) \
		   $(TEXBITS) $(BIBBITS) \
		   Makefile

###############################################################################

# Some comments about some of the `DVIPSFLAGS' and `PS2PDFFLAGS'.
#
# -Pdownload35 --- Embed the standard PostScript fonts.  The USENIX author
# instructions (and many other conference instructions) ask that *all* fonts be
# embedded in PDF documents.  Note that you *must* use this option in order for
# `ps2pdf14' to produce working PDF.  Note that the the name of the embedded
# `Times' font is called `Nimbus'.  (See the `ps2pk.map' file.)
#
# -u ps2pk.map --- I think this is not required, but it doesn't hurt.  I think
# `dvips' consults it anyway.  I could be wrong; maybe it is required in some
# cases.
#
# -d... --- For the `ps2pdf' options the deal with font embedding, I believe
# that all of these are the standard values for modern versions of Ghostscript
# (7.05+).
#
# `PS2PDFFLAGS' and `PS2PDFFLAGS_EPS' used to include "-dUseCIEColor".  This
# was removed because modern versions of Ghostscript warn:
#
# > Use of -dUseCIEColor detected!
# > Since the release of version 9.11 of Ghostscript we recommend you do not
# > set -dUseCIEColor with the pdfwrite/ps2write device family.
#
# Now we use "-dColorConversionStrategy=/RGB -dProcessColorModel=/DeviceRGB".
#
# Note that you can use the `pdffonts' tool to check that all the fonts are
# embedded.
#
# Some random but handy URLs for these things:
#   <http://www.crhc.uiuc.edu/~mjmille2/howtos/latex-howtos/>
#   <http://www.cs.wisc.edu/~ghost/doc/gnu/7.05/Ps2pdf.htm>

###############################################################################

.DELETE_ON_ERROR:

.PHONY: all clean realclean
all::
clean::
realclean::

###############################################################################

all:: $(DOC)

define def-doc-rule
  .PHONY: $1
  $1: $1.pdf
endef
$(foreach d,$(DOCUMENTS),$(eval $(call def-doc-rule,$d)))

.PHONY: ps
ps: $(DOC)-ps.ps

.PHONY: pdf
pdf: $(DOC).pdf

define def-ps-pdf-rule
  $1-ps.pdf: $1-ps.ps
	$$(PS2PDF) $$(PS2PDFFLAGS) $$<
endef
$(foreach d,$(DOCUMENTS),$(eval $(call def-ps-pdf-rule,$d)))

.PHONY: html
html: $(DOC)-www.html

define def-www-rule
  $1-www.html: $1-www.dvi
	$$(TEX4HT) $$(basename $$@)
	$$(T4HT) $$(basename $$@)
endef
# And if you have `wwwis' <http://bloodyeck.com/wwwis/>,
#	wwwis *.html
$(foreach d,$(DOCUMENTS),$(eval $(call def-www-rule,$d)))

####

$(addsuffix .pdf,$(DOCUMENTS)): $(DEPS) $(FIGPDF)
$(addsuffix -ps.dvi,$(DOCUMENTS)): $(DEPS) $(FIGEPS)
$(addsuffix -www.dvi,$(DOCUMENTS)): $(DEPS) $(FIGWWW)

# Why be subtle?
# Use a special job name to keep our output docs separate from those along the
# "normal" route to PDF.
%-ps.dvi: %.tex
	$(LATEX) -jobname $(basename $@) $(basename $<)
	- $(BIBTEX) $(basename $@)
	$(LATEX) -jobname $(basename $@) $(basename $<)
	$(LATEX) -jobname $(basename $@) $(basename $<)
#	$(LATEX) -jobname $(basename $@) $(basename $<)

%-www.dvi: %-www.tex
	$(LATEX) -jobname $(basename $@) $(basename $<)
	- $(BIBTEX) $(basename $@)
	$(LATEX) -jobname $(basename $@) $(basename $<)
	$(LATEX) -jobname $(basename $@) $(basename $<)
#	$(LATEX) -jobname $(basename $@) $(basename $<)

%.ps: %.dvi
	$(DVIPS) $(DVIPSFLAGS) $(basename $@) -o $@

# Why be subtle?
%.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) -draftmode $(basename $<)
	- $(BIBTEX) $(basename $@)
	$(PDFLATEX) $(PDFLATEXFLAGS) -draftmode $(basename $<)
	$(PDFLATEX) $(PDFLATEXFLAGS) $(basename $<)
#	$(PDFLATEX) $(PDFLATEXFLAGS) $(basename $<)

%.bbl: %.aux
	$(BIBTEX) $(basename $@)

####

%.eps: %.fig
	$(FIG2DEV) -L eps $< $@

# ENE: I think this is the "old way," but I'm not sure.
# %.pdf: %.fig
#	$(FIG2DEV) -L pdf $< $@

# Be careful to apply this rule only to FIGBITS.  Some of our figures may come
# from other sources, and generate EPS and PDF versions on their own.
$(FIGBITS:.fig=.pdf): %.pdf: %.eps
	$(PS2PDF) $(PS2PDFFLAGS_EPS) $< $@
# The "old way" does not embed the fonts:
#	$(EPSTOPDF) $<

# "-m 1.5 -S 4": magnify and smooth
%.png: %.fig
	$(FIG2DEV) -L png -m 1.5 -S 4 $< $@

####

%.eps: %.svg
	$(INKSCAPE) \
	$< \
	--export-eps=$@

%.pdf: %.svg
	$(INKSCAPE) \
	$< \
	-D --export-pdf=$@

%.png: %.svg
	$(INKSCAPE) \
	$< \
	-D --export-png=$@

%.eps: %.gnu
	$(GNUPLOT) \
	$<

# This method produces small PDFs that have tight bounding boxes.
$(PLOTBITS:.gnu=.pdf): %.pdf: %.eps
	$(PS2PDF) $(PS2PDFFLAGS_EPS) $< $@

# NOTES
#
# First: if we seriously cared about EPS as a terminal format, we would want to
# add `--export-text-to-path' to the command line:
#
# %.eps: %.svg
# 	$(INKSCAPE) \
# 	$< \
# 	--export-eps=$@ \
# 	--export-text-to-path
#
# Second, Inkscape's `--export-to-pdf' feature does work all that well.  So we
# use a different method.

# This method produces small PDFs that have tight bounding boxes.
# $(SVGBITS:.svg=.pdf): %.pdf: %.eps
#	$(PS2PDF) $(PS2PDFFLAGS_EPS) $< $@

###############################################################################

## How to build the various plots with gnuplot.
##
## The rules in this section express the custom dependencies between the plots,
## the scripts that generate them, and the data files that the scripts read.
## Some scripts generate more than one plot when they are run.  Some plots
## read more than one data file.  The names of the various files are somewhat
## ad hoc, so we need custom rules to express the dependencies.
##
## In each rule, the script is the first dependency.  This allows the action
## of every rule to be exactly the same.  Almost.

## E.g.,
#
# figs/crashes_by_size.eps: \
# 		code/crashes_by_size.gp \
# 		code/crashes_by_size_bar.txt
# 	cd figs && env GNUPLOT_LIB="../code" $(GNUPLOT) $(notdir $<)

# $(GNUPLOTPDF): %.pdf: %.eps
#	$(PS2PDF) $(PS2PDFFLAGS_EPS) $< $@

###############################################################################

## How to build the set of things required for the final VEE 2016 submission
## package.

.PHONY: vee
vee: $(VEE_PDF) $(VEE_TEX)
# vee: $(VEE_PDF) $(VEE_PS) $(VEE_TEX)

$(VEE_PDF): submit.pdf
	$(CP) $< $@

## ENE: Sheridan no longer requires a PS file; hooray!
#
# I had hoped to generate the PS version using the usual DVI->PS process, but
# this does not work.  It fails because we use the `microtype' package, which
# leads to different typesetting between the PDF and DVI outputs of `pdflatex'.
#
# $(VEE_PS): submit-ps.ps
# 	$(CP) $< $@
#
# So now we take the cheesy... er, easy way out.  We produce PS from PDF!
#
# Do *not* use `pdf2ps' (from the Ghostscript package) for this conversion.
# That tool turns all the fonts into bitmaps.  Instead, use `pdftops' (from the
# Xpdf/Poppler package).  The `pdftops' tool retains T1 fonts and in addition
# makes a smaller file.
#
# $(VEE_PS): submit.pdf
#	$(PDFTOPS) $< $@

# The submission metadata LaTeX file.
$(VEE_TEX): $(addsuffix .m4,$(VEE_TEX)) \
	header.tex \
	abstract.tex \
	submit.bbl

%.tex: %.tex.m4
	$(M4) --prefix-builtins $< > $@

###############################################################################

clean::
	$(RM) *.aux *.bbl *.blg *.dvi *.log *.out
	$(RM) *-www.4ct *-www.4tc *-www.idv *-www.lg *-www.tmp *-www.xref \
	      tex4ht.fls

realclean:: clean
	$(RM) *.eps *.pdf *.ps
	$(RM) *-www.css *-www*.html *-www*.png
	$(RM) $(VEE_TEX)
	$(RM) $(FIGBITS:.fig=.eps) $(SVGBITS:.svg=.eps) $(GNUPLOTEPS) \
		$(PLOTBITS:.gnu=.eps)
	$(RM) $(FIGBITS:.fig=.pdf) $(SVGBITS:.svg=.pdf) $(GNUPLOTPDF) \
		$(PLOTBITS:.gnu=.pdf)
	$(RM) $(FIGBITS:.fig=.png) $(SVGBITS:.svg=.png) $(GNUPLOTWWW) \
		$(PLOTBITS:.gnu=.png)

###############################################################################

## End of file.

